Spatio-temporal Person Retrieval via Natural Language Queries

In this paper, we address the problem of spatio-temporal person retrieval from multiple videos using a natural language query, in which we output a tube (i.e., a sequence of bounding boxes) which encloses the person described by the query. For this problem, we introduce a novel dataset consisting of videos containing people annotated with bounding boxes for each second and with five natural language descriptions. To retrieve the tube of the person described by a given natural language query, we design a model that combines methods for spatio-temporal human detection and multimodal retrieval. We conduct comprehensive experiments to compare a variety of tube and text representations and multimodal retrieval methods, and present a strong baseline in this task as well as demonstrate the efficacy of our tube representation and multimodal feature embedding technique. Finally, we demonstrate the versatility of our model by applying it to two other important tasks.

==> Makefile <==
.SUFFIXES: .tex .dvi .aux .log .toc .lof .lot .pdf .ps .bbl .bib .blg
F=paper_for_review
SUP=sup_for_review
FIN=paper_final
FINSUP=sup_final
# F=paper_final
TEX=platex
CHAPTER=$(shell ls *.tex)
CHAPAUX=$(shell ls *.aux)

all: $F.pdf
	open $F.pdf
	./send_server.sh
	touch $F.tex
# 	ls chapters_eng/*tex | xargs -n1 grammar-check | grep -v WHITESPACE_RULE | grep -v WHITESPACE_RULE COMMA_PARENTHESIS_WHITESPACE | grep -v WHITESPACE_RULE | grep -v EN_QUOTES | grep -v CURRENCY

sup: ${SUP}.pdf
	open ${SUP}.pdf
	./send_server.sh

final: ${FIN}.pdf
	open ${FIN}.pdf

supfinal: ${FINSUP}.pdf
	open ${FINSUP}.pdf

pdf: $F.pdf
dvi: $F.dvi
bbl: $F.bbl
ps:  $F.ps

$F.dvi:$F.tex $F.bbl $(CHAPTER)
#$F.dvi:$F.tex $(CHAPTER)
$F.pdf:$F.dvi
$F.ps:$F.dvi
$F.bbl:$F.bib
$F.aux:$F.tex

${SUP}.dvi:${SUP}.tex ${SUP}.bbl $F.bbl
${SUP}.pdf:${SUP}.dvi
${SUP}.ps:${SUP}.dvi
${SUP}.bbl:${SUP}.bib
${SUP}.aux:${SUP}.tex

${FIN}.dvi:${FIN}.tex ${FIN}.bbl
${FIN}.pdf:${FIN}.dvi
${FIN}.ps:${FIN}.dvi
${FIN}.bbl:${FIN}.bib
${FIN}.aux:${FIN}.tex

${FINSUP}.dvi:${FINSUP}.tex ${FINSUP}.bbl
${FINSUP}.pdf:${FINSUP}.dvi
${FINSUP}.ps:${FINSUP}.dvi
${FINSUP}.bbl:${SUP}.bib
${FINSUP}.aux:${FINSUP}.tex

.dvi.ps:
#	dvips -t a4 -Ppdf -o $@ $*
	dvips -Ppdf -o $@ $*
.dvi.pdf:
	dvipdfmx $*
#	pdflatex -shell-escape $F.tex

.bib.bbl:
	${TEX} $*; pbibtex $*; platex $*; platex $*;

.tex.aux:
	$(TEX) $*

clean:
	rm -f *~ $F.dvi $F.aux $F.lof $F.toc $F.lot $F.log \
               $F.pdf $F.ps $F.bbl $F.blg
	rm -f $(CHAPAUX) *.pbm

cleanwopdf:
	rm -f *~ $F.dvi $F.aux $F.lof $F.toc $F.lot $F.log \
               $F.ps $F.bbl $F.blg
	rm -f $(CHAPAUX) *.pbm

cleansup:
	rm -f *~ ${SUP}.dvi ${SUP}.aux ${SUP}.lof ${SUP}.toc ${SUP}.lot ${SUP}.log \
               ${SUP}.ps ${SUP}.bbl ${SUP}.blg
	rm -f $(CHAPAUX) *.pbm

